Logarithmic Regret in Feature-based Dynamic Pricing

Feature-based dynamic pricing is an increasingly popular model of setting prices for highly differentiated products with applications in digital marketing, online sales, real estate and so on. The problem was formally studied as an online learning problem [Javanmard & Nazerzadeh, 2019] where a seller needs to propose prices on the fly for a sequence of $T$ products based on their features $x$ while having a small regret relative to the best -- "omniscient" -- pricing strategy she could have come up with in hindsight. We revisit this problem and provide two algorithms (EMLP and ONSP) for stochastic and adversarial feature settings, respectively, and prove the optimal $O(d\log{T})$ regret bounds for both. In comparison, the best existing results are $O\left(\min\left\{\frac{1}{\lambda_{\min}^2}\log{T}, \sqrt{T}\right\}\right)$ and $O(T^{2/3})$ respectively, with $\lambda_{\min}$ being the smallest eigenvalue of $\mathbb{E}[xx^T]$ that could be arbitrarily close to $0$. We also prove an $\Omega(\sqrt{T})$ information-theoretic lower bound for a slightly more general setting, which demonstrates that "knowing-the-demand-curve" leads to an exponential improvement in feature-based dynamic pricing.

==> log_checklist_neurips21.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% Checklist %%%%%%%%%%%%%%%%%%%%%%%%

\section*{Checklist}
\begin{comment}
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\end{comment}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{ We summarized our main contribution in Section \ref{sec_introduction} ``Summary of Results'' part. In order to support these results, we rigorously specified the problem settings, present corresponding algorithms and their theoretical analysis as well as numerical experiments.}
  \item Did you describe the limitations of your work?
    \answerYes{In Section \ref{sec_discussion}, we carefully discussed a number of problems that are still open after our results being present, including noises, modeling, coefficients, etc. In Appendix \ref{appendix_sec_more_discussion}, we further showed details of these issues.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{In Appendix \ref{appendix_ethic}, we talked about some ethic issues including pricing discriminations and privacies. However, these are all naturally existing issues, and our algorithms would not worsen the cases. In fact, the online dynamic pricing problem we considered in this work can also be viewed as an online auction problem, which would improve market efficiency and help both buyers and sellers to identify the right prices with less exploration.}
    	
%    	definitely reduce pricing discriminations as the prices are public to all customers.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{In the numerical experiments, we only used simulated data that has nothing to do with the natural sciences and do not include human subjects. The paper is theoretical in nature and the purpose of the numerical simulation is to validate the theoretical predictions.}
  	
%    	For the other parts of this paper, we totally conducted theoretical analysis. }
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{We stated three basic assumptions in Section \ref{sec_preliminary} ``Summary of Assumptions''. We later stated Assumptions \ref{random_iid_xt} and \ref{assumption_fixed_unknown_parameter} for specific theorems.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{We completely proved every claim we made. In fact, our paper and appendices are filled with proofs.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We included all codes and data in the supplementary material, along with a ``Readme'' document as instructions of running the program and reproduce our results. }
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Actually we did not pre-train the algorithms as we considered online learning problems. However, we did specify the hyperparameters and the way they were chosen, in Section \ref{sec_num_result} and Figure \ref{fig:plots}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report all error bars and error bands with 0.95 coverage using Wald's test.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{We just ran all numerical experiments on a laptop. We did mention that the experiment of EXP-4 is very time-consuming. However, this is because EXP-4 is actually an exponential time algorithm, and in fact EXP-4 is an existing algorithm instead of our contributions.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{We did not use existing assets.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not use crowdsourcing or conduct research with human subjects.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> proof_adversarial/ONSP_regret_analysis.tex <==
In this section, we present the regret analysis of Algorithm \ref{algo_ONSP}. Primarily, we propose the main theorem.

\begin{theorem}\label{theorem_ONSP_main}
    With Assumptions \ref{assumption_gaussian_noise_iid}, \ref{assumption_convex_feature_and_parameter_set}, \ref{assumption_bounded_x_set}, the regret of Algorithm \ref{algo_ONSP} (ONSP) satisfies:
    \begin{equation}
        Reg_{Alg_{\ref{algo_ONSP}}}\leq C_{a}(B,\sigma)\cdot d\log{T},
        \label{equation_ONSP_regret}
    \end{equation}
    where $C_{a}(B,\sigma)$ is a function that only depends on $B$ and $\sigma$.
\end{theorem}

Similar to that in Section \ref{sec_random}, we divide the proof of Theorem \ref{theorem_ONSP_main} into 2 parts: (1) we upper bound the regret by the regret of expected likelihood function; (2) since ONSP takes likelihood function as a (surrogate) loss function, we can upper bound the regret of likelihood according to the principle of online Newton method. 

Specifically, denote $u_t^*:=x_t^T\theta^{*}, u_t:=x_t^T\theta_{t}, J(u_t)=v_t$, and we have the following Theorems.

\begin{theorem}\label{thmupb}
    \begin{equation*}
	g(J(u_t^*),u_t^{*})-g(J(u_t),u_t^{*})\leq C_2\cdot\E_{N_t}[l_t(\theta_{t})-l_t(\theta^{*})],
	\end{equation*}
	where $C_2=2\cdot\frac{0.6+\frac{B^2}{4\sigma^2}}{C_{down}}$.
\end{theorem}

The proof of Theorem \ref{thmupb} is similar to that of Theorem \ref{theorem_surrogate} in Section \ref{sec_random}. Please find the detailed proof in Appendix \ref{adv_append_proof_of_surrogate_loss}. With Theorem \ref{thmupb}, we may reduce the regret of likelihood functions as a surrogate regret of pricing. From Lemma \ref{strong_convexity} we see that the log-likelihood function is $\frac{C_{down}}{C_{exp}}$-exponentially concave, which enables us to apply Online Newton Step method to achieve a logarithmic regret. Therefore, by citing from Online Convex Optimization \citep{hazan2019introduction}, we have the following Theorem.%Also, we cite the other theorem from \citet{hazan2019introduction} Theorem 4.4:

\begin{theorem}\label{thmons} With parameters $\gamma = \frac{1}{2}\min\{\frac{1}{4GD}, \alpha\}$ and $\epsilon=\frac{1}{\gamma^2D^2}$, and $T>4$ guarantees:
	\begin{equation*}
	\sup_{\{x_t\}}\left\{\sum_{t=1}^{T}l_t(\theta_{t})-\min_{\theta\in\mathbb{H}}\sum_{t=1}^{T}l_t(\theta)\right\}\leq5\left(\frac{1}{\alpha}+GD\right)d\log T.
	\end{equation*}
	Here $\alpha = \frac{C_{down}}{C_{exp}}$, $D=2\cdot B_1$ and $G=\frac{p_{\sigma}(3B+2\sigma)}{1-\Phi_{\sigma}(3B+2\sigma)}\cdot B_2$.
\end{theorem}

With Theorem \ref{thmupb} and \ref{thmons}, we have:
\begin{equation}
\begin{aligned}
Reg=&\sum_{t=1}^{T}\left(g(J(u_t^*),u_t^{*})-\E_{N_1, N_2, \ldots, N_{t-1}}[g(J(u_t),u_t^{*})]\right)\\
\leq&\sum_{t=1}^{T}\left(C_2\cdot\E_{N_1, N_2, \ldots, N_{t-1}}[\E_{N_t}[l_t(\theta_t)-l_t(\theta^{*})]]\right)\\
\leq&C_2\cdot\E_{N_1, N_2, \ldots, N_{t-1}}[\E_{N_t}[\sum_{t=1}^{T}l_t(\theta_t)-\min_{\theta\in\Omega}\sum_{t=1}^{T}l_t(\theta)]]\\
\leq&C_2\cdot5\left(\frac{1}{\alpha}+GD\right)d\log T.
\end{aligned}
\end{equation}
Therefore, we have proved Theorem \ref{theorem_ONSP_main}. {$\blacksquare$}

